TCM-Eval: An Expert-Level Dynamic and Extensible Benchmark for Traditional Chinese Medicine

Large Language Models (LLMs) have demonstrated remarkable capabilities in modern medicine, yet their application in Traditional Chinese Medicine (TCM) remains severely limited by the absence of standardized benchmarks and the scarcity of high-quality training data. To address these challenges, we introduce TCM-Eval, the first dynamic and extensible benchmark for TCM, meticulously curated from national medical licensing examinations and validated by TCM experts. Furthermore, we construct a large-scale training corpus and propose Self-Iterative Chain-of-Thought Enhancement (SI-CoTE) to autonomously enrich question-answer pairs with validated reasoning chains through rejection sampling, establishing a virtuous cycle of data and model co-evolution. Using this enriched training data, we develop ZhiMingTang (ZMT), a state-of-the-art LLM specifically designed for TCM, which significantly exceeds the passing threshold for human practitioners. To encourage future research and development, we release a public leaderboard, fostering community engagement and continuous improvement.

==> section/4_method.tex <==

% 在本节，我们将详细的描述我们如何基于在Section 3中精心收集的TCMBench训练集，在Deepseek-R1的基础上进行后训练，我们的核心思想是利用拒绝采样算法使模型自我迭代进化，同时我们利用deepseek-r1本身的思考能力，对仅包含问题、答案的二元组 (Q, A)，结合人工辅助标注出了高质量思维链数据 (Q, T, A)，其中Q、T、A分别代表问题、思考过程和答案。

% 具体来说，我们把初始的部分训练集都输入给初始的Deepseek-R1，记作M_0，然后我们过滤掉那些错误的回答，保留回答正确的答案，并把其中的思维链加入训练集，紧接着我们继续把这部分错误的回答输入给M_0，再次把正确的回答加入思维链，最后我们把模型一直答错的题目交给专业的医学团队，基于人工标注出正确的思考过程，基于此我们构建出了第一批带有正确思考过程的数据集，我们对M_0进行SFT得到M_1，紧接着我们继续此过程，直到把所有的训练集都完整训练一遍，得到我们的最终模型ZhiMingTang。基于此方法，我们仅需极少的人工标注过程，即可利用QA pair来实现思考模型自我迭代式的进化。

\section{SI-CoTE} \label{sec:method}
This section details our proposed \textbf{Self-Iterative Chain-of-Thought Enhancement (SI-CoTE)} framework for training the \textbf{ZhiMingTang}. The framework is built upon the Deepseek-R1 \cite{guo2025deepseek} base model, denoted as $\mathcal{M}_0$. At its core, the SI-CoTE methodology employs a phased, iterative process to efficiently convert the original Question-Answer (QA) pair dataset, $\mathcal{D}_{\text{QA}}$, into an enhanced dataset containing high-quality CoT data, thereby driving the evolution of the model's capabilities.

Initially, we partition the original QA dataset into $K$ disjoint subsets:

\begin{equation}
    \mathcal{D}_{\text{QA}} = \mathcal{D}_1 \cup \mathcal{D}_2 \cup \dots \cup \mathcal{D}_K
    \label{eq:partition}
\end{equation}

Our training process then unfolds iteratively over these subsets. In the $k$-th iteration (for $k=1, \dots, K$), we focus on generating high-quality CoT for the QA pairs $(Q_i, A_i^*) \in \mathcal{D}_k$.

Specifically, in the $k$-th iteration, we leverage the model from the previous iteration, $\mathcal{M}_{k-1}$, where $\mathcal{M}_0$ is the initial base model, to generate candidate CoT and answer pairs $(T_i, A_i)$ for each question $Q_i$ in subset $\mathcal{D}_k$. The generated answers are then filtered using a verification function. This \textbf{Rejection Sampling} step retains a candidate if and only if its generated answer $A_i$ is consistent with the ground-truth answer $A_i^*$. This condition is formally expressed as:

\begin{equation}
    V(A_i, A_i^*) = 1
    \label{eq:verification}
\end{equation}

For questions where the model fails to produce a correct answer after multiple attempts, these "hard cases" are identified and annotated with high-quality CoT by medical experts. Through this combined approach of machine generation-verification and human-in-the-loop assistance, we construct a high-quality CoT dataset, $\mathcal{D}_{\text{CoT}, k}$, for the corresponding data subset $\mathcal{D}_k$.

The key to this framework lies in the accumulation of data and the iterative evolution of the model. The newly generated CoT data from each iteration is aggregated into a cumulative SFT training set. At the conclusion of the $k$-th iteration, this set is updated as follows:

\begin{equation}
    \mathcal{D}_{\text{SFT}}^{(k)} = \bigcup_{j=1}^k \mathcal{D}_{\text{CoT}, j}
    \label{eq:update_sft}
\end{equation}

We then fine-tune the base model $\mathcal{M}_0$ on this continuously expanding and refined dataset to yield a more capable next-generation model, $\mathcal{M}_k$:

\begin{equation}
    \mathcal{M}_k = \text{SFT}(\mathcal{M}_0, \mathcal{D}_{\text{SFT}}^{(k)})
    \label{eq:finetune}
\end{equation}

Having learned the reasoning patterns from the first $k$ subsets, the enhanced model $\mathcal{M}_k$ exhibits stronger reasoning capabilities and a higher success rate when processing the subsequent subset, $\mathcal{D}_{k+1}$. This process continues until all $K$ subsets have been processed. The final model, \textbf{ZhiMingTang}, denoted as $\mathcal{M}_K$, is trained on the complete, high-quality CoT dataset $\mathcal{D}_{\text{SFT}}^{(K)}$. Through this batch-wise, iterative enhancement approach, the SI-CoTE framework achieves a synergistic evolution of model capability and data quality.
